Goal-Driven Explainable Clustering via Language Descriptions

Unsupervised clustering is widely used to explore large corpora, but existing formulations neither consider the users' goals nor explain clusters' meanings. We propose a new task formulation, "Goal-Driven Clustering with Explanations" (GoalEx), which represents both the goal and the explanations as free-form language descriptions. For example, to categorize the errors made by a summarization system, the input to GoalEx is a corpus of annotator-written comments for system-generated summaries and a goal description "cluster the comments based on why the annotators think the summary is imperfect.''; the outputs are text clusters each with an explanation ("this cluster mentions that the summary misses important context information."), which relates to the goal and precisely explain which comments should (not) belong to a cluster. To tackle GoalEx, we prompt a language model with "[corpus subset] + [goal] + Brainstorm a list of explanations each representing a cluster."; then we classify whether each sample belongs to a cluster based on its explanation; finally, we use integer linear programming to select a subset of candidate clusters to cover most samples while minimizing overlaps. Under both automatic and human evaluation on corpora with or without labels, our method produces more accurate and goal-related explanations than prior methods. We release our data and implementation at https://github.com/ZihanWangKi/GoalEx.

==> old_appllication.tex <==

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{CluGE-product.pdf}
    \caption{Example taxonomy for complaints about beauty products from Amazon \citep{he2016ups}. }
    \label{fig:product}
\end{figure*}

\section{Applications} \label{sec:application}
We adapted \methodname{} to construct taxonomies by hierarchically generating finer-grained clusters.
We present qualitative findings, discuss the limitations of our system, and point out future directions.

\subsection{Hierarchical Applications of \methodname{}} \label{sec:recursive-method}
How does \methodname{} work in more realistic applications beyond diagnostic benchmarks? We apply \methodname{} on 

\begin{itemize}[topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,leftmargin=2em]
  \item  human-written feedback for model-generated summaries \cite{scheurer2023training}, with the goal of ``\textit{categorizing model errors},
  \item debates on why spanking is bad, with the goal of ``\textit{categorizing the types of arguments}'' \cite{habernal-gurevych-2016-makes}, and
  \item 1-star Amazon reviews \citep{he2016ups} under the Beauty category, with the goal of  ``\textit{categorizing customer complaints}''.
\end{itemize}

For every output cluster with more than 20 samples, we apply \methodname{} again to create finer-grained clusters and output trees of explanations as taxonomies;
when creating child clusters for a parent cluster, we include the explanation for the parent cluster into the original goal and request the new candidate explanations to be sub-categories of the parent's explanation. 
Here is an example goal where the parent's explanation is in \textbf{bold}:

\noindent ``\textit{My goal is to cluster feedback for model-generated summaries. Now we have gathered the feedback that fall under the following category: \textbf{whether this feedback advises adding omitted details; specifically, the feedback points out that certain key details or aspects are missing from the text, which is necessary for a complete understanding. For example, 'The summary should include specific details about why things in their day went wrong.'}, and I want to create finer-grained cluster descriptions that fall under the above category.}''

We set $K = 8$, $\lambda = 0.5$, proposer $=$ \texttt{gpt-4} \citep{openai2023gpt4}, and assigner $=$ \texttt{Claude-v1.3} \citep{bai2022constitutional}. 
We allow a sample to appear in multiple clusters so that \methodname{} can see as many samples as possible when creating subcategories.
We additionally designed a new prompt template to propose more detailed explanations; see Appendix Figure \ref{fig:proposal-complex} for more details.


\subsection{Qualitative Analysis} \label{sec:qualitative-analysis}

\noindent \textbf{Outputs of \methodname{}.}
Even though we have only attempted depth-2 taxonomy in this paper, an entire taxonomy can contain up to $8^2=64$ explanations, which are impossible to fit in this paper.    
Therefore, we display a subset of representative explanations and common error patterns in the main paper, report the coverage and overlaps for the first round of \methodname{}, and include the full taxonomies in our github.

Figure \ref{fig:demo} shows representative explanations for model errors; 75\% of the samples are supported by at least one explanation, while 10\% of the samples are assigned to more than one cluster.
Figure \ref{fig:spanking} shows representative explanations for arguments against spanking; 83\% are supported, while 2\% have overlap.
Figure \ref{fig:product} shows representative explanations for customer complaints; 59\% are supported, while 14\% have overlap. 

\noindent \textbf{Analysis.} Across the three applications, we found that many explanations adhere to the goal and plausibly describe sub-parts of the given corpus. 
Compared to previous algorithms, \methodname{} can cluster texts in a goal-driven way, and the explanations could help the users quickly explore the corpus without inspecting each cluster manually.

\noindent \textbf{Limitations and Future Work.} On the other hand, however, many samples are not supported by any cluster; the reason might be that the proposer is still incapable of identifying all minority clusters, or eight clusters are inherently insufficient to cover all samples. 
Future work could improve the proposal stage to better recover small clusters and adaptively decide the appropriate number of clusters. 

The explanations also sometimes do not form a coherent taxonomy. 
For example, as shown in Figure \ref{fig:spanking}, the explanation ``\textit{employs rhetorical questions}'' is irrelevant to the goal of identifying argument types;
additionally, the explanation ``\textit{discusses the cycle of violence}'' appears both in the first and second levels of the taxonomy and hence should be merged.
Future work could improve the proposer's ability to generate explanations that are more goal-related and resolve the redundancy of explanations at a global level.
Given these weaknesses, the practitioner should still be responsible for properly interpreting the results of \methodname{}.

Additionally, reaching the best performance requires using \texttt{gpt-4} and \texttt{claude-v1.3} as the proposer and the assigner, which might induce a large cost via LM APIs if one needs to run \methodname{} on a large corpus; we hope such a problem would alleviate in the future if we could use a lighter weight model to approximate the assigner, the cost of computation significantly decreases, or there is a more computationally efficient variant of \methodname{}.
